Automata and Fixpoints for Asynchronous Hyperproperties

Hyperproperties have received increasing attention in the last decade due to their importance e.g. for security analyses. Past approaches have focussed on synchronous analyses, i.e. techniques in which different paths are compared lockstepwise. In this paper, we systematically study asynchronous analyses for hyperproperties by introducing both a novel automata model (Alternating Asynchronous Parity Automata) and the temporal fixpoint calculus $\Hmu$, the first fixpoint calculus that can systematically express hyperproperties in an asynchronous manner and at the same time subsumes the existing logic HyperLTL. We show that the expressive power of both models coincides over fixed path assignments. The high expressive power of both models is evidenced by the fact that decision problems of interest are highly undecidable, i.e. not even arithmetical. As a remedy, we propose approximative analyses for both models that also induce natural decidable fragments.

==> math/defs/criticality.tex <==
\begin{definition}[Criticality]
	For a $H_{\mu}$ formula $\varphi$ in positive normal we denote with criticality the number of critical quantifiers along any path from root to leaf in the formula's syntax tree.
	A quantifier is called critical iff at least one of the following conditions applies:
	\begin{enumerate}
		\item it is an existential quantifier preceded by a universal quantifier
		\item it is a universal quantifier preceded by an existential quantifier
		\item it is the outermost quantifier in scope of a fixpoint expression
	\end{enumerate}
\end{definition}

==> math/defs/existentialuniversalfragment.tex <==
\begin{definition}
	We say that a $H_{\mu}$ formula is in the existential (resp. universal) fragment, if there are no universal (resp. existential) quantifiers and $\land$ (resp. $\lor$) constructs in its positive normal form.
\end{definition}

==> math/defs/noisy.tex <==
\begin{definition}
	We call a language $\mathcal{L} \subseteq (\Sigma^n)^{\omega}$ \textit{noisy} in component $d \leq n$, if the following condition holds:
	for all $w \in (\Sigma^n)^{\omega}$ and $v \in \Sigma^{\omega}$ we have $w \in \mathcal{L}$ iff $w[v / d] \in \mathcal{L}$.
\end{definition}

==> math/defs/omegasynchronous.tex <==
\begin{definition}
A formula of H$_\mu$ is called $\omega$-\textit{synchronous} if
\end{definition}


==> math/defs/parityholes.tex <==
Let $\Sigma$ be an input alphabet.
An Alternating Parity Automaton (APA) is a tuple 
$\mathcal{A} = (Q, q_0, \rho, \Omega)$
such that 
\begin{itemize}
\item $Q$ is a finite, non-empty set of control locations,
\item $q_0 \in Q$ is an initial control location,
\item $\rho: Q \times \Sigma \rightarrow \mathcal{B}^+(Q)$ is a function that maps control locations and input symbols
to positive boolean formulas over control locations and
\item $\Omega: Q  \rightarrow \{0, 1, \dots k\}$ is a function that maps control locations to priorities.
\end{itemize}

==> math/proofs/aapaclosure.tex <==
\begin{proof}
For union and intersection, use a boolean combination of the starting functions to glue the automata together.
For complement, shift priorities by one and swap $\land/\lor$ transitions in $\rho_0$ and $\rho$.
%\hfill\qed
\end{proof}

==> math/proofs/aapahmuequivalence.tex <==
\begin{proof}
	For 1): Similar construction as in \cite{Bozzelli2007}.
	Directions are added in the following way: all nodes of the form $\bigcirc_i$ have direction $i$, all other nodes have direction $-$.
	Proof of correctness is done in a similar way by intermediate automata over the alphabet $S^n \times \varrho \times \mathbb{N}_0^n$ (where $\varrho$ is the set of all path predicate environments $\rho$) with holes $X_i$ for free path predicates $X_i$.
	
	For 2): 
	Fix an AAPA $\mathcal{A} = (Q, q_0, \rho, \Omega)$. 
	We inductively construct formulae $\varphi^h_i$. 
	%Let $\rho(q_h, a) = \bigvee C_i$ with $C_i = \bigwedge (q_{i_k}, r_{i_k})$. 
	We set $\varphi^h_0 \equiv \bigvee_{a \in \Sigma} (\bigwedge a_i \land \hat{\rho}(q_h, a))$ such that $\hat{\rho}(q_h, a)$ is the formula obtained by replacing each entry $q_j$ by $\bigcirc_k X_j$ if if $\delta(q_h) = k$ and by $X_j$ if $\delta(q_h) = -$. 
	Furthermore, for $i > 0$ and $h = i$, we set $\varphi_i^i \equiv \mu X_i. \varphi_{i-1}^i$ if $ \Omega(q_i)$ is odd and $\varphi_i^i \equiv \nu X_i. \varphi_{i-1}^i$ if $ \Omega(q_i)$ otherwise. \dots
	%\qed\hfill
\end{proof}

\begin{comment}
$\mathcal{A_{\varphi}} = (sub(\varphi),(\varphi),\rho,\Omega,\delta)$ with
\begin{itemize}
\item $\rho(a_i, \mathpzc{s}) = (true), a_i \in L(w_i)$,
\item $\rho(\neg a_i, \mathpzc{s}) = (true), a_i \notin L(w_i)$,
\item $\rho(\varphi_1 \land \varphi_2, \mathpzc{s}) = (\varphi_1) \land (\varphi_2)$
\item $\rho(\varphi_1 \lor \varphi_2, \mathpzc{s}) = (\varphi_1) \lor (\varphi_2)$
\item $\rho(\langle \cdot \rangle_i \psi, \mathpzc{s}) = (\psi)$
\item $\rho(\mu X. \psi, \mathpzc{s}) = (\psi)$
\item $\rho(\nu X. \psi, \mathpzc{s}) = (\psi)$
\item $\rho(X, \mathpzc{s}) = (\psi_X)$
\item $\Omega(X) = 2 \cdot f_{pd}(\varphi) - (2 \cdot f_{pd}(\varphi_X) - 1)$ if $\varphi_X$ is a $\mu$ formula
\item $\Omega(X) = 2 \cdot f_{pd}(\varphi) - 2 \cdot f_{pd}(\varphi_X)$ if $\varphi_X$ is a $\nu$ formula
\item $\Omega(\psi) = 2 \cdot f_{pd}(\varphi)$ if $\psi \neq X$
\item $\delta(\bigcirc_i \psi) = i$
\item $\delta(\psi) = -$ if $\psi \neq \bigcirc_i$
\end{itemize}
\end{comment}

==> math/proofs/aapatechnicallemma.tex <==
\begin{proof}
	Let $\mathcal{A}$ be an AAPA recognising some language $\mathcal{L}$ which is noisy in component $d$.
	$\mathcal{A}'$ is obtained from $\mathcal{A}$ by substituting direction $d$ with $-$ in every state.
	Now if $\sigma \in \Sigma$ is the first letter in component $d$ of some word $w$, then a run of $\mathcal{A}'$ on $w$ exactly corresponds to a run of $\mathcal{A}$ on $w[\sigma^{\omega} / d]$.
	We show that $\mathcal{A}'$ recognises $\mathcal{L}$.
	Therefore let $w \in \Sigma^{\omega}$ be a word and $\sigma \in \Sigma$ be the first letter in component $d$ of $w$.
	On the one hand assume that $w \in \mathcal{L}$.
	From the fact that $\mathcal{L}$ is noisy in component $d$, we have that $w[\sigma^{\omega} / d] \in \mathcal{L}$.
	Since $\mathcal{A}$ recognises $\mathcal{L}$, we have an accepting run of $\mathcal{A}$ on $w[\sigma^{\omega} / d]$, which from the above argument exactly corresponds to a run of $\mathcal{A}'$ on $w$ witnessing $w \in \mathcal{L}(\mathcal{A}')$.
	On the other hand assume that $w \in \mathcal{L}(\mathcal{A}')$.
	By the above argument, its run exactly corresponds to a run of $\mathcal{A}$ on $w[\sigma^{\omega} / d]$, which recognises $w[\sigma^{\omega} / d] \in \mathcal{L}(\mathcal{A}) = \mathcal{L}$.
	Since $\mathcal{L}$ is noisy in component $d$, we then have $w \in \mathcal{L}$.
\end{proof}

==> math/proofs/alternatingcomparison.tex <==
\begin{proof}
	The proof is by induction on $d$.
	
	In the \textbf{base case}, the formula is given as $\psi_{\mathcal{A}}(\pi,\pi')$ where $\mathcal{A}$ is the automaton from \autoref{lem:phaseboundedcomparison}.
	
	For the \textbf{inductive step}, we assume that phases in $\psi_{diff}^{d,k}(\pi_1,\pi_2)$ start with $\pi_1$.
	The automaton in \autoref{lem:phaseboundedcomparison} was constructed in a way that this is the case.
	This way we can ensure that no more than $k$ index switches are made.
	We construct the inductive formula as follows:
	\begin{align*}
		\psi_{diff}^{d+1,k}(\pi,\pi') := &\ \forall \pi_{index} . \psi_{stock}^{d-1,k}(\pi_{index}) \rightarrow \\
		& (\mathcal{G}_{\pi} \psi_{diff}^{d,k}(\pi,\pi_{index}) \lor \lnot ie_{\pi} \mathcal{U}_{\pi} 1_{\pi} \land \\
		& \mathcal{G}_{\pi'} \psi_{diff}^{d,k}(\pi',\pi_{index}) \lor \lnot ie_{\pi'} \mathcal{U}_{\pi'} 0_{\pi'}) \lor \\
		& (\mathcal{G}_{\pi} \psi_{diff}^{d,k}(\pi,\pi_{index}) \lor \lnot ie_{\pi} \mathcal{U}_{\pi} 0_{\pi} \land \\
		& \mathcal{G}_{\pi'} \psi_{diff}^{d,k}(\pi',\pi_{index}) \lor \lnot ie_{\pi'} \mathcal{U}_{\pi'} 1_{\pi'})
	\end{align*}
	Note that $\psi_{diff}$ only occurs in such a way that no further context switches are made.
\end{proof}

==> math/proofs/alternatingexpressivity.tex <==
\begin{proof}
AAPAs are closed under intersection while NAPAs are not.
%\hfill\qed
\end{proof}

==> math/proofs/alternatingstockmeyer.tex <==
\begin{proof}
	$\psi_{stock}^{d,k}(\pi)$ makes use of a variation of $\psi_{td}^{d,k}(\pi)$ with languages:
	\begin{align*}
		\mathcal{L}_1^{td} :=&\ \{0^n | n \in \mathbb{N}_0\} \\
		\mathcal{L}_2^{td} :=&\ \{1^n | n \in \mathbb{N}_0\} \\
		td :=&\ \{ (w,w') \in (\{0,1\}^n)^2 | n \in \mathbb{N}_0, w' = w + 1\}
	\end{align*}
	In addition, it checks whether starting and ending symbol of a word are the brackets belonging to the respective level.
	Markers separating the words are brackets indicating the beginning and end of a level $d + k - 1$ encoded index.
	%and skips bits belonging to the encoded word while doing the transductions for additions, i.e. the transductions are only performed on indices in the encoding.
\end{proof}

==> math/proofs/alternatingtransducer.tex <==
\begin{proof}
	Proof by induction on $d$.
	
	\textbf{Base case:}
	\begin{align*}
	\psi_{td}^{0,k}(\pi) :=\ & \exists \pi' . \psi_{\mathcal{A}}(\pi,\pi')
	\end{align*}
	for the AAPA $\mathcal{A}$ from \autoref{lem:phaseboundedtransducer}.
	
	\textbf{Inductive step:}
	\begin{align*}
	\psi_{td}^{d+1,k}(\pi) :=\ & \forall \pi_{index}. \psi_{stock}^{d-1,k}(\pi_{index}) \rightarrow \\
	& \mathcal{G}_{\pi} \psi_{stock}^{d,k}(\pi) \land \\
	& \psi_{start}^{d,k}(\pi) \land \mathcal{F}_{\pi} \psi_{final}^{d,k}(\pi) \land\\
	& \mathcal{G}_{\pi} \psi_{diff}^{d,k}(\pi,\pi_{index}) \lor \\
	&\bigvee_{b \in \{0,1\}} \lnot ie_{\pi} \mathcal{U}_{\pi} b_{\pi} \land \\
	&\psi_{diff}^{d,k}(\pi,\pi_{index}) \mathcal{U}_{\pi} (\lnot ie_{\pi} \mathcal{U}_{\pi} td(b)_{\pi})
	\end{align*}
	\tbd{If $\psi_{diff}$ contains quantifiers and occurs inside a modality, the quantifiers cant be moved into a prenex form}
	\begin{align*}
	\psi_{td}^{d+1,k}(\pi) :=\ &\exists \pi_{ref} \forall \pi_{conf} . \psi_{stock}^{d,k}(\pi_{conf}) \rightarrow \\
	& \text{Startkonfiguration in } \pi \text{ und}\\
	& \text{Endkonfiguration in } \pi \text{ und}\\
	& \text{Wenn } \pi_{conf} \text{ in } \pi \text{ dann auch Nachfolger oder }\\
	& \pi_{conf} \text{ ist Endkonfiguration}
	\end{align*}
	\tbd{Make sure no phases are added.
	Idea: no use of $\psi_{td}^{d,k}$ from induction hypothesis inside modalities.
	This also makes sure quantifiers can be used in prenex form.}
\end{proof}

==> math/proofs/analyticalhierarchy.tex <==
\begin{proof}
Hardness follows from \autoref{thm:aapasigmaone} and \autoref{thm:aapahmuequivalence}.
For inclusion, we proceed as follows: For every quantifier, we use an additional input vector consisting of an alternating stream of $0$ and $1$ for every atomic proposition. Then, for an existential quantifier, we always existentially guess an assignment of atomic propositions. This can be done by asynchronously advancing in the vectors. At every step, we can also ensure that the guess is actually a valid path prefix of the Kripke model. 
For universal quantifiers, we use conjunctive alternation for the streams. For path prefixes which are not actually possible in the structure, we immediately move into an accepting state with a self-loop in order to accept. 
The language of the resulting automaton is non-empty iff the formula is fulfilled by the structure.
\end{proof}



==> math/proofs/appahmuequivalence.tex <==
\begin{proof}
Fix an AAPA $\mathcal{A} = (Q, q_0, \rho, \Omega)$.
We inductively construct formulae $\phi^h_i$. 
We set $\phi^h_0 = \bigvee_{a \in \Sigma} (\bigwedge a_i \land \hat{\rho(q_h, a)}$ such that $\hat{\rho(q_h, a)} = \bigwedge \delta(X_j)$ where
$\delta(X_j) = \bigcirc_j X_j$ ... and $X_j$ otherwise.
\end{proof}



==> math/proofs/asynchronousCTL.tex <==
\begin{proof}
All cases are immediate except the asynchronous modalities.
We translate them as follows:
\begin{itemize}
\item $Tr(\phi_1 \mathcal{U} \exists \phi_2) = \exists \pi_1 \exists^1 \pi_2 F^1 ((\exists^2 \pi_3 (Tr(\phi_1) \land F^3 (sync(\pi_1) \land Tr(\phi_2))\mathcal{U}^2 sync(\pi_1, \pi_2)$
\item $Tr(\phi_1 \mathcal{U} \forall \phi_2) = \exists \pi_1 \exists^1 \pi_2 \forall^2 \pi_3 F^1 (Tr(\phi_1) \mathcal{U}^3 Tr(\phi_2)$
\end{itemize}
\end{proof}
\tbd{Repair this proof:  Brackets in second case don't match; Whcih semantics of the translation matches semantics of CTL+sync?}


==> math/proofs/asynchronousexpressivity.tex <==
\begin{proof}
	The language $\mathcal{L}$ is given as $\{(a,a,a)^n(b,a,a)^n (b,b,a)^n (b,b,b)^{\omega} | n \in \mathbb{N}\}$.
	A NAPA $\mathcal{A}$ can recognize the language by moving one step in component 1, two steps in component 2, and three steps in component 3 at a time reading $a$s and then moving to an accepting or rejecting cycle reading $b$s in all components depending on whether all components reached a $b$ at the same time.
	For the other claim we show that $\mathcal{L}$ is not recognized by a pushdown automaton.
	This is however not the case since the prefix $(a,a,a)^n (b,a,a)^n (b,b,a)^n$ is clearly not context-free.	
	%\hfill\qed
\end{proof}

==> math/proofs/boundedsynchronousemptiness.tex <==
\begin{proof}
For fixed $n$, the APA from our remark only has polynomial size implying PSPACE membership.
For hardness, notice that every APA can be seen as a synchronous AAPA, yielding a reduction from he emptiness problem for APAs.
\end{proof}

==> math/proofs/continuity.tex <==
\begin{proof}
Let  $\Pi$ be a path assignment and $e_i$ be the $i$th unit vector. Let $p_1(c_1, \dots, c_n, a) = (c_0, \dots, c_n)$ be the projection onto the first $n$ components and $p_2$ be the projection onto the last component. Finally, set $A = \{1 \dots n\}$, $A' = A \cup \{-\}$ and $M =  \mathbb{N}^n \times A'$. Define the \textit{asynchronous unfolding} to be the Kripke structure $\mathcal{AU}(\Pi) = (S, s_0, \delta, L)$ with $S =\mathbb{N}^n \times A$, $s_0 = (0, \dots, 0, -)$, 
$\delta(m) = \{m' \in M \mid \exists a \in A : p_1(m') = p_1(m) + e_a \land p_2(m') = a\}$. Finally, set $L(c_0, \dots, c_n, a) = \bigcup L(\pi_i (c_i)) \cup \{step_a\}$. 
Intuitively, $AU$ glues together all paths in single nodes such that each node is is connected with those nodes that represent an asynchronous advancement by one step from the origin. The labels are transferred from the individual paths to the node and the node is additionally labelled with the direction of the last advancement. $\mathcal{AU}$ has a branching degree of $n$ and is thus finitely branching.
A path formula $\psi$ of H$_\mu$ can be translated into a formula $\hat{\psi}$ of the modal $\mu$-calculus by replacing formulae $\bigcirc_{\pi_i} \psi'$ by $\langle \rangle (psi' \land step_i)$ inductively.
By simultaneous induction on the structure of $\varphi$, we can show two claims: 1)  $(c_1, \dots, c_n) \in  \llbracket \varphi \rrbracket^{\mathcal{V}}_k(\Pi)$ iff $(c_1, \dots, c_n, a) \in [\hat{\phi}]$ for some $a \in A$ and
2) if $v \in \llbracket \varphi \rrbracket^{\mathcal{V}}_k(\Pi)$, then there is 
Since the semantics of the modal $\mu$-calculus is continuous on finitely branching structures, Kleene's fixpoint theorem implies $(c_1, \dots, c_n) \in g(\xi)$.
Furthermore, we can show using induction and Kleenes's fixpoint theorem that if $(c_1, \dots, c_n) \in g(\xi)$
\end{proof} 
\tbd{Notation anpassen und Stetigkeit präzise folgern}


==> math/proofs/existentialmodelchecking.tex <==
\begin{proof}
	
\end{proof}

==> math/proofs/existentialsigmaone.tex <==
\begin{proof}
By \autoref{thm:aapahmuequivalence}, there is a existential $H_{\mu}$ formula $\phi_{\mathcal{A}}$ for every AAPA $\mathcal{A}$ such that $\phi_{\mathcal{A}}$ is satisfiable iff $\mathcal{A}$ is non-empty. By \autoref{thm:aapasigmaone}, the latter problem is $\Sigma_1^1$-complete.  
\end{proof}


==> math/proofs/existsforallsatisfiability.tex <==
\begin{proof}
For membership in 2EXPSPACE, we can use the same argument as for HyperLTL and translate a formula $\varphi$ into a $\forall^*$-formula of exponential size and test it for satisfiability in EXPSPACE. 
For hardness, we reduce from the satisfiability problem for $\Sigma_3$ QPTL formulae which is 2EXPSPACE-complete.
Let $\varphi \equiv \exists a_1 \dots a_k \forall a_1' \dots a_m' \exists a_1'' \dots a_n'' \psi$ be a $\Sigma_3$ QPTL formula where $\psi$ is an LTL formula. (There can actually be unboundedly many quantifiers...)
For $\psi$, we construct an Alternating (synchronous) Büchi Automaton (ABA) $\mathcal{A}$ in the standard way. However, instead of accepting sets of atomic propositions as input symbols, we augment $\mathcal{A}$ with an input vector that contains an entry for every atomic proposition. These entries together represent the trace.
However, the entries for $a_1'' \dots a_n''$ actually consist of atomic propositions and alternative choices for these propositions.
Then, whenever we take a transition in $\mathcal{A}$, we either use the current input bit or asynchronously switch to the next input bit before that for each of those entries. This modification turns $\mathcal{A}$ into a 2-synchronous AAPA.
Replacing $\mathcal{A}$ by the formula $\varphi_{\mathcal{A}}$ in $H_{\mu}$, we obtain the $H_{\mu}$ formula $\psi \equiv \exists \pi_{a_1} \dots \pi_{a_k} \exists \pi_{a_1''} \dots \exists \pi_{a_n''} \forall \pi_{a_1'} \dots \pi_{a_m'}
\varphi_{\mathcal{A}} \land \varphi_{zo}$ where $\varphi_{zo} \equiv \bigwedge_{d=1}^n a_{\pi_{a_d''}} \land \mathcal{G} (a_{\pi_{a_d''}} \rightarrow \bigcirc \neg a_{\pi_{a_d''}} \land \neg a_{\pi_{a_d''}} \rightarrow \bigcirc a_{\pi_{a_d''}})$ and $a$ is the atomic proposition that matches the atomic proposition of each entry when equipped with the corresponding path index.
This formula is equisatisfiable to $\varphi$.
\end{proof}


==> math/proofs/hyperpdl.tex <==
\begin{proof}
	Since HyperPDL-$\Delta$ is defined on Kripke Transition Systems and $H_{\mu}$ is defined on Kripke Structures, we have to bring them to a common ground.
	We therefore extend $H_{\mu}$ to Kripke Transition Systems by replacing $\bigcirc \varphi$ with $\langle \sigma \rangle \varphi$.
	This does however not change the expressivity of $H_{\mu}$ since $\langle \sigma \rangle \varphi$ can easily be encoded by $\bigcirc (\sigma \land \bigcirc \varphi)$ in the setting where a Kripke Transition System is translated back to a Kripke Structure via elimination of transition labels by intermediate states.
	
	$tr_{\varphi}: HyperPDL-\Delta \to H_{\mu}$
	\begin{align*}
		\exists \pi. \varphi' &\mapsto \exists \pi . tr_{\varphi}(\varphi') \\
		\forall \pi. \varphi' &\mapsto \forall \pi . tr_{\varphi}(\varphi') \\
		a_{\pi_i} &\mapsto a_i \\
		\lnot \varphi' &\mapsto \lnot tr_{\varphi}(\varphi') \\
		\varphi' \lor \varphi'' &\mapsto tr_{\varphi}(\varphi') \lor tr_{\varphi}(\varphi'') \\
		\varphi' \land \varphi'' &\mapsto tr_{\varphi}(\varphi') \land tr_{\varphi}(\varphi'') \\
		\langle \alpha' \rangle \varphi' &\mapsto tr_{\alpha}(\alpha')(tr_{\varphi}(\varphi')) \\
		[\alpha'] \varphi' &\mapsto \lnot tr_{\varphi}(\langle \alpha' \rangle \lnot \varphi') \\
		\Delta \alpha' &\mapsto \nu X . tr_{\alpha}(\alpha')(X)
	\end{align*}
	
	$tr_{\alpha}: \alpha \to H_{\mu}(x)$ where $x$ can be seen as a nonterminal in the grammar for $H_{\mu}$. $tr(\alpha)(\varphi)$ is then $tr(\alpha)$ with all occurrences of $x$ replaced by $\varphi$. Note that $\varphi$ can introduce new nonterminals $x$.
	\begin{align*}
		\tau &\mapsto \langle \tau|_1 \rangle_1 ... \langle \tau|_n \rangle x \\
		\varepsilon &\mapsto x \\
		\alpha_1 \alpha_2 &\mapsto tr_{\alpha}(\alpha_1)(tr_{\alpha}(\alpha_2))\\
		\alpha_1 + \alpha_2 &\mapsto tr_{\alpha} (\alpha_1) \lor tr_{\alpha} (\alpha_2) \\
		\alpha_1^* &\mapsto \mu X. x \lor tr_{\alpha}(\alpha_1)(X) \\
		\varphi ? &\mapsto tr_{\varphi}(\varphi)
	\end{align*}
	%\hfill\qed
\end{proof}

==> math/proofs/ksynchronousdecidability.tex <==
\begin{proof}
Since $H_{\mu}$ model checking is undecidable,
we can reduce an instance $\langle M,w \rangle$ of the halting problem to the question whether a Kripke structure $\mathcal{K}$ fulfills a $H_{\mu}$ formula $\varphi_{M,w}$.
Fix a $k$-synchronous formula $\varphi$ and a formula $\varphi'$ that is not $k$-synchronous for any $k \in \mathbb{N}_0$ when evaluated on $\mathcal{K}$ such that $\mathcal{K} \models \varphi \leftrightarrow \neg \varphi'$. 
Furthermore, we can construct a formula $Char(\mathcal{K})$ (even in the $\mu$-calculus or CTL) with the property that $\mathcal{K}' \models Char(\mathcal{K})$ iff the structure $\mathcal{K}'$ is bisimilar to $\mathcal{K}$. Then $\psi_{M,w} \equiv Char(\mathcal{K}) \land (\varphi_{M, w} \rightarrow \varphi) \land (\neg \varphi_{M,w} \rightarrow \varphi')$ is semantically equivalent to a $k$-synchronous formula iff $\mathcal{K} \models \varphi_{M,w}$. 
This induces a reduction from $H_{\mu}$ model checking to the question under consideration.
%\hfill\qed
\end{proof}

==> math/proofs/ksynchronoussatisfiability.tex <==
\begin{proof}
	An $\exists^*$ $H_{\mu}$ formula $\varphi$ is satisfiable, iff the automaton $\mathcal{A}_{\varphi}$ from \autoref{thm:aapahmuequivalence} is non-empty.
	Using complementation, one can obtain a similar result for the $\forall^*$ fragment.
	For $k$-synchronous formulae, $\mathcal{A}_{\varphi}$ is a $k$-synchronous AAPA, thus transformable into an equivalent APA of exponential size by \autoref{thm:aapaksynchronoustosynchronous}.
	Since emptiness tests on APAs can be performed in PSPACE, we obtain an EXPSPACE algorithm.
	Using, the other direction of \autoref{thm:aapahmuequivalence}, a $k$-synchronous AAPA $\mathcal{A}$ can be transformed into a quantifier-free $k$-synchronous $H_{\mu}$ formula $\varphi_{\mathcal{A}}$ of (asymptotically) the same size such that $\mathcal{A}$ is non-empty iff $\exists \pi_1 ... \exists \pi_n \varphi_{\mathcal{A}}$ is satisfiable.
	Since the emptiness problem for $k$-synchronous AAPAs is EXPSPACE-complete, we obtain a lower bound.
\end{proof}

==> math/proofs/linearphaseboundedmodelchecking.tex <==
\begin{proof}
The upper bound follows from \autoref{thm:constructionsize} and the NLOGSPACE complexity of emptiness tests on NPAs.

For hardness, we use an argument similar to the one in the proof of \autoref{thm:ksynchronousmodelchecking}.
This time, we build a $k$ phase-bounded AAPA as in the proof of \autoref{cor:phaseboundedcomplexity} that checks whether the word between two propositions represents a correct encoding of a $k$-exponentially long word and build a corresponding quantifier alternation free $H_\mu$ formula for it.
The inductive construction as for HxperLTL does however not preserve phase-boundedness since a trivial translation of synchronous advancement leads to a phase switch after every step.
\tbd{Adapt inductive construction}
\end{proof}


==> math/proofs/modelchecking.tex <==
\begin{proof}
Encode two NAPAs over the alphabet $\Sigma^2$ by formulae $\psi_1$ and $\psi_2$ with free path variables $\pi_1$ and $\pi_2$.
For a model $\mathcal{K}$ with $Traces(\mathcal{K}) = \Sigma^{\omega}$, $\mathcal{K} \models \exists \pi_1 . \exists \pi_2 . \psi_1 \land \psi_2$ iff the intersection of the NAPAs is non-empty. 
%\hfill\qed
\end{proof}

==> math/proofs/mucalculus.tex <==
\begin{proof}
	$tr: L_{\mu} \to H_\mu$
	\begin{equation*}
		\varphi \mapsto \exists \pi_1 . \hat{tr}(\varphi, 1)
	\end{equation*}
	$\hat{tr}: L_{\mu} \times \mathbb{N} \to H_\mu$
	\begin{align*}
		\hat{tr}(p,i) &= p_i \\
		\hat{tr}(X,i) &= X \\
		\hat{tr}(\bigcirc_i \varphi,i) &= \exists \pi_{i+1} . \bigcirc_{i+1} \hat{tr}(\varphi,i+1) \\
		\hat{tr}(\varphi \lor \varphi',i) &= \hat{tr}(\varphi,i) \lor \hat{tr}(\varphi',i) \\
		\hat{tr}(\lnot \varphi,i) &= \lnot \hat{tr}(\varphi,i) \\
		\hat{tr}(\mu X. \varphi,i) &= \mu X. \hat{tr}(\varphi,i)
	\end{align*}
\end{proof}

==> math/proofs/paritydealternation.tex <==
\begin{proof}
	For 1):
	The idea here is to remove holes while storing their information in the input alphabet, then applying a standard alternation removal algorithm to finally restore information about holes from the input alphabet into a function $h$.
	Therefore we swtich input alphabets from $\Sigma$ to $\Sigma \times 2^{\{X_1,...,X_m\}}$, where in a word $w = (w_0,\chi_0)(w_1,\chi_1)... \in (\Sigma \times 2^{\{X_1,...,X_m\}})^{\omega}$, $X_i \in \chi_j$ implies $w_j w_{j+1} ... \in \mathcal{L}(\mathcal{A}_i)$.
	
	Holes are removed one by one in the following way:
	When eliminating $X_i$ we go over from $\hat{\Sigma}$ to $\hat{\Sigma} \times 2^{\{X_i\}}$.
	For each state $q \in Q$ and each letter $\sigma \in \hat{\Sigma}$, we divide $\rho(q,\sigma)$ into two parts $\rho_{X_i}(q,\sigma)$ and $\rho_{\emptyset}(q,\sigma)$, the first one describing exactly the valuations making $X_i$ true to satisfy $\rho(q,\sigma)$ and the second one describing exactly those making $X_i$ false to satisfy $\rho(q,\sigma)$.
	We manipulate $\rho_{X_i}(q,\sigma)$ in such a way that $X_i$ is removed from all valuations while maintaining the truth values of all other atoms.
	Then we chose $\rho(q,(\sigma,\{X_i\})) := \rho_{X_i}(q,\sigma)$ and $\rho(q,(\sigma,\emptyset)) := \rho_{\emptyset}(q,\sigma)$.
	Now all runs of $\mathcal{A}$ on some $w \in \hat{\Sigma}^{\omega}$ that had $X_i$ on levels $j_1,j_2,...$ have a corresponding run where exactly $w_{j_1},w_{j_2},...$ are extended with $\{X_i\}$ and all other letters are extended with $\emptyset$.
	
	After the elimination of all holes, we obtain an automaton $\mathcal{A}_h$ without holes which accepts a word $w \in (\Sigma \times 2^{\{X_1,...,X_m\}})^{\omega}$ iff each letter $w_i$ contains exactly the holes on level $i$ of an acceptin run of $\mathcal{A}$ on $w$'s projection to $\Sigma^{\omega}$.
	We use a standard alternation elimination algorithm to obtain a nondeterministic Büchi automaton $\mathcal{A}'$ with $2^{\mathcal{O}(n \cdot k \cdot log\ n)}$ states recognizing the same language.
	
	We split each state of $\mathcal{A}'$ into $2^m$ copies, one for each $\chi \in 2^{\{X_1,...,X_m\}}$ such that all incoming transitions share the same second component.
	Since all $m$ holes are states in $\mathcal{A}$, we have $m \leq n$ and this state split does not asymptotically increase the size of $\mathcal{A}'$.
	The marking function $h$ is then chosen in such a way that $h(q) = \chi$ where $\chi$ is the set of holes all incoming transitions into $q$ are sharing in their second component.
	At this point we can switch input alphabets back to $\Sigma$ again by removing the $\chi$ component of all transitions and joining the transition sets now sharing the same letter again, that is: $\rho(q,\sigma) = \bigcup_{\chi \in 2^{\{X_1,...,X_m\}}} \rho(q,(\sigma,\chi))$.
	
	We obtain the desired equivalence in the following way:
	Let $w = w_0 w_1 ... \in \Sigma^{\omega}$. 
	Then:
	\begin{align*}
		&w \in \mathcal{L}(\mathcal{A}[X_1 : \mathcal{A}_1,...,X_m : \mathcal{A}_m]) \\
		\text{iff }
		&\mathcal{A}[X_1 : \mathcal{A}_1,...,X_m : \mathcal{A}_m] \text{ has an accepting run on } w \\
		\text{iff }
		&\mathcal{A} \text{ has an accepting run on } w \text{ where } X_i \text{ on level } j \\
		&\text{ implies } w_j w_{j+1} ... \in \mathcal{L}(\mathcal{A}_i) \\
		\text{iff }
		&\mathcal{A}_h \text{ has an accepting run on } (w_0,\chi_0)(w_1,\chi_1)... \\
		&\text{ where } X_i \in \chi_j \text{ implies } w_j w_{j+1} ... \in \mathcal{L}(\mathcal{A}_i) \\
		\text{iff }
		&\mathcal{A}' \text{ has an accepting run on } (w_0,\chi_0)(w_1,\chi_1)... \\
		&\text{ where } X_i \in \chi_j \text{ implies } w_j w_{j+1} ... \in \mathcal{L}(\mathcal{A}_i) \\
		\text{iff } 
		&\mathcal{A}' \text{has an accepting run } q_0' q_1' ... \text{ om } w \text{ such that } \\
		&X_i \in h(q_j') \text{ implies } w_j w_{j+1} ... \in \mathcal{L}(\mathcal{A}_i)
	\end{align*}
	For 2):
	Straightforward switch of disjunctive and conjunctive transitions and shift of priorities by one.
	%\hfill\qed
\end{proof}

	
\begin{comment}
Let $\mathcal{A} = (Q,q_0,\rho,\Omega)$ be an APA.
We construct an NPA $\mathcal{A}' = (Q',q_0',\rho',\Omega')$ with the same amount of priorities.
The set of states $Q'$ is given as $(2^Q)^k \times \{0,1\}$ and we write states as $(Q_1,...,Q_k)_c$.
Intuitively, a state $(Q_1,...,Q_k)_c$ tracks information of a level in $\mathcal{A}$s runtree $T$, where a state $q \in Q_i$ means that there is a branch in $T$ that is in state $q$ on the tracked level and has seen $i$ as the lowest priority so far.
The index $c$ is a tag indicating whether the lowest even priority has been visited on each branch in $T$ yet.
Thus the starting state $q_0'$ is a state where $Q_i = \{q_0\}$ with $i = \Omega(q_0)$ and $Q_j = \emptyset$ for $j \neq i$ tagged with $0$.
We choose $\Omega'$ in the following way: In all untagged states we have $\Omega'((Q_1,...,Q_k)_0) = 3$. 
%is the greatest odd $j$ such that $Q_j \neq \emptyset$, if it exists, and the greatest even $j$ such that $Q_j \neq \emptyset$, else.
In all tagged states we have $\Omega'((Q_1,...,Q_k)_1) = 1$, if there is an odd $j$ with $Q_j \neq \emptyset$ and $\Omega'((Q_1,...,Q_k)_1) = 2$ else.
Hereby we ensure that only those states have an even priority where the lowest priority seen on each branch is even.
Last, we have to construct $\rho'$ such that states $(Q_1,...,Q_k)_c$ match our intuition.
This is done in the following way: $\rho'((Q_1,...,Q_k)_c,\sigma) = \bigvee_{c'\geq c}(Q_1',...,Q_k')_{c'}$ with $Q_i' = \{q \in \rho(Q_j,\sigma) | (j > i \land \Omega(q) = i) \lor (j = i \land \Omega(q) \geq i)\}$ where $\rho(Q_j,\sigma) = \bigcup\{\{q_1,...,q_l\} \subseteq Q | \{q_1,...,q_l\} \models \rho(q,\sigma) \text{ for some } q \in Q_j\}$.

We now show that $\mathcal{A}$ and $\mathcal{A}'$ indeed recognize the same language.
On the one hand assume that $w \in \mathcal{A}$.
By definition there is an accepting run $T$ of $w$ on $\mathcal{A}$ where the lowest priority occuring on each path starting in the root is even.
From this we construct an accepting run $q_0 q_1 ...$ of $w$ on $\mathcal{A}'$: $q_m = (Q_1,...,Q_k)$ is constructed from level $m$ of $T$ such that $Q_i = \{q \in Q | \exists t \in T. |t| = m \land r(t) = q \land min\{\Omega(r(t')) | t' \in \pi_t\} = i\}$.
It is straightforward to see that $q_{l+1} \in \rho'(q_l,w(l))$ from the fact that (i) when node $t$ has children $t_1,...,t_l$, then $\{r(t_1),...,r(t_l)\} \models \rho(r(t),w(|t|))$, and (ii) states are sorted by the lowest priority seen so far in $\pi_{t_i}$.
From (ii) it is also straightforward to see that the lowest priority on $q_0 q_1 ...$ is even since all paths in $T$ starting at $\varepsilon$ have an even lowest priority.
Thus at some point all states will be sorted into sets with even priorities.
It is not possible
\end{comment}

==> math/proofs/pushdownexpressivity.tex <==
\begin{proof}
	We choose an alphabet with three letters $a$, $b$ and $\bot$.
	The language $\mathcal{L}$ is such that the first component starts with $a^n b^n \bot$.
	After that and in all other components any combination of letters is allowed.
	A Büchi Pushdown can easily recognise the language by just inspecting the start of the first component.
	The other claim follows from an intuitive but rather technical result about asynchronous automata: when a language containing only \textit{noise} in one direction is recognised by some asynchronous automaton, then there is another asynchronous automaton recognising the same language without inspecting that direction.
	We refer the interested reader to the appendix for a proof of this claim.
	Thus we can assume, that an AAPA recognising $\mathcal{L}$ only moves forward in the first direction and therefore behaves like an APA.
	Then the claim follows from the fact that $a^n b^n$ is a non-regular prefix.
\end{proof}

==> math/proofs/satisfiability.tex <==
\begin{proof}
	Encode two NAPAs over the alphabet $\Sigma^2$ by formulae $\psi_1$ and $\psi_2$ with free path variables $\pi_1$ and $\pi_2$.
	Then $\exists \pi_1 . \exists \pi_2 . \psi_1 \land \psi_2$ is satisfiable iff the intersection of the NAPAs is non-empty.
\end{proof}
\begin{comment}
\begin{proof}
Hardness follows from \autoref{thm:analyticalhierarchy} since we can encode Kripke structures in the standard way. 
For inclusion, a non-deterministic Büchi TM can guess a tree satisfying a formula $\varphi$ iff the formula is satisfiable.
\end{proof}
\end{comment}
\begin{comment}
Translate the polyadic $\mu$-calculus into $H_\mu$.
%\hfill\qed
\end{comment}


==> math/proofs/syncexistsforallsatisfiability.tex <==
\begin{proof}
	We transform a synchronous $\exists^* \forall^*$ $H_{\mu}^{sync}$ formula into a synchronous $\exists^*$ $H_{\mu}^{sync}$ formula of exponential size using the same arguments as for $\exists^* \forall^*$ HyperLTL satisfiability.
	Since satisfiability for alternation-free synchronous $H_{\mu}^{sync}$ is in PSPACE, we obtain an EXPSPACE algorithm for the problem at hand.
	For hardness, we reduce from $\exists^* \forall^*$ satisfiability for HyperLTL, which is EXPSPACE-complete.
	The translation of a HyperLTL formula into an equivalent $H_{\mu}$ formula is straightforward and introduces a polynomial blowup at most, yielding the reduction.
\end{proof}

==> math/proofs/synchronoussatisfiability.tex <==
\begin{proof}
	Transform a universally quantified formula $\varphi$ into a formula $\varphi'$ of the linear time $\mu$-calculus by removing trace variables, then test $\varphi'$ for satisfiability in PSPACE.
	Since $\varphi$ is equisatisfiable to $\varphi$, we can negate an existentially quantified formula and apply a validity check for the linear time $\mu$-calculus that runs in PSPACE.
	The lower bound in both cases follows from the corresponding lower bound for that logic.  
	%\hfill\qed
\end{proof}


==> math/theorems/aapamultipushdown.tex <==
\begin{theorem}
	The emptiness problem for $k$ phase-bounded AAPAs can be decided in $2(k-1)$EXPTIME.
\end{theorem}

\tbd{Direkt multi-queue systems benutzen? Evtl. sogar 1 bzw 2EXPTIME}

\begin{proof}
	We reduce the emptiness problem on $k$ phase-bounded AAPAs to the problem of solving a $2(k-1)$ phase bounded multi-pushdown parity game.
	The reduction is done in two steps.
	First the AAPA is converted to an alternating multi-queue parity automaton, which is then converted to an alternating multi-pushdown parity automaton, which can be interpreted as a parity game, where a winning strategy corresponds to an accepting run of the automaton.
	
	For the first step, we use a queue for each component of the input alphabet.
	When reading an input vector, each symbol is enqueued into its corresponding queue.
	Transitions are then calculated from each of the front elements.
	when encountering a direction, a dequeue operation is performed on the corresponding queue.
	A phase of the AAPA is then transformed into a phase of the multi-queue automaton, where dequeue operations are only allowed on a single queue.
	The first phase of the AAPA does however form an exception, since here, symbols in the associated direction can directly be read from the input.
	
	For the second step, we simulate each queue of the multi-queue automaton by two stacks, where one stack handles enqueue- and one stack handles dequeue operations.
	The idea is that one of the stacks holds the entire content of the queue while the other one is empty.
	Enqueue operations then correspond to push operations on the enqueue stack while that stack holds the content of the queue.
	When a dequeue operation follows, the queue's content is moved from one stack to the other one element at a time.
	Therefore a phase switch in the multi-queue automaton needs two phases in the multi-pushdown automaton: one phase to switch the old queue from dequeue to enqueue mode and one phase to switch the new queue from enqueue to dequeue mode.
	
	Finally, the alternating multi-pushdown parity automaton can be converted to a parity game, where $\lor$-transitions correspond to player $0$ choices, $\land$-transitions correspond to player $1$ choices and a winning strategy for player $0$ induces an accepting run.
	%\hfill\qed
\end{proof}

==> math/theorems/aapatechnicallemma.tex <==
\begin{lemma}
	Let $\Sigma^n$ be an asynchronous alphabet and $d \leq n$ a direction.
	Let $\mathcal{L}$ be a language which is noisy in component $d$ and recognised by an AAPA $\mathcal{A}$.
	Then there is an AAPA $\mathcal{A}'$ recognising $\mathcal{L}$ without moving forward in direction $d$.
\end{lemma}

==> math/theorems/alternatingcomparison.tex <==
\begin{lemma}\label{lem:alternatingcomparison}
	Given a size bound $m$, there is a $k$ phase-bounded alternation depth $d$ $H_{\mu}$ formula $\psi_{diff}^{d,k}(\pi,\pi')$ of size polynomial in $m$ that expresses that the level $d + k - 1$ encoded words of length $g(d + k - 1, m)$ in $\pi$ and $\pi'$ differ.
\end{lemma}

==> math/theorems/alternatingstockmeyer.tex <==
\begin{lemma}\label{lem:alternatingstockmeyer}
	Given a size bound $m$, there is a $k$ phase-bounded alternation depth $d$ $H_{\mu}$ formula $\psi_{stock}^{k,d}(\pi)$ of size polynomial in $m$ that expresses that $\pi$ is level $d + k$ nested index encoded.
\end{lemma}

==> math/theorems/alternatingtransducer.tex <==
\begin{lemma}\label{lem:alternatingtransducer}
	Given a size bound $m$, there is a $k$ phase-bounded alternation depth $d$ $H_{\mu}$ formula $\psi_{td}^{d,k}(\pi)$ of size polynomial in $m$ which expresses that $\pi$ contains a sequence of level $d+k-1$ encoded words $w_1 w_2 ... w_l$, each of length $g(d+k-1,m)$, separated by markers, such that
	\begin{itemize}
		\item $w_1$ is contained in a given regular language $\mathcal{L}_1^{td}$ with an acceptor of size $\mathcal{O}(m)$
		\item $w_l$ is contained in another given regular language $\mathcal{L}_2^{td}$ with an acceptor of size $\mathcal{O}(m)$
		\item for $i < l$, $w_{i+1}$ is obtained from $w_{i}$ by applying the regular transducer $td$ of size $\mathcal{O}(m)$.
	\end{itemize}
\end{lemma}

==> math/theorems/analyticalhierarchy.tex <==
\begin{theorem}\label{thm:analyticalhierarchy}
The model checking problem of the $\Delta_n$ fragment of H$_\mu$ against a finite Kripke model is $\Pi^1_1$-complete
\end{theorem}



==> math/theorems/asynchronousCTL.tex <==
\begin{theorem}
CTL+Sync \cite{Chatterjee2016} can be embedded into $H_{\mu}^{sync}$.
\end{theorem}


==> math/theorems/asynchronousexpressivity.tex <==
\begin{theorem}
There is a language $\mathcal{L}$ such that there is a NAPA $\mathcal{A}$ with $\mathcal{L}(\mathcal{A}) = \mathcal{L}$ while no Büchi pushdown automaton can recognize $\mathcal{L}$.
\end{theorem}


==> math/theorems/asynchronousmodelchecking.tex <==
\begin{theorem}
	Model Checking a $k$ phase-bounded $H_{\mu}$ formula from the $\forall^*$ or $\exists^*$ fragment is decidable in $2kEXPTIME$.
\end{theorem}

==> math/theorems/existentialmodelchecking.tex <==
\begin{theorem}
	Model Checking a $H_{\mu}$ formula from the existential or universal fragment is decidable in PSPACE.
\end{theorem}

==> math/theorems/existentialsigmaone.tex <==
\begin{theorem}
The emptiness problem for the $\exists^*$ and $\forall^*$-fragment of $H_{\mu}$ is $\Sigma_1^1$-complete.
\end{theorem}


==> math/theorems/existsforallsatisfiability.tex <==
\begin{theorem}
The satisfiability problem for the $k$-synchronous $\exists^* \forall^*$-fragment of $H_{\mu}$ is 2EXPSPACE-complete.
\end{theorem}


==> math/theorems/hmutoaapasize.tex <==
\begin{theorem}
	The automaton $\mathcal{A}_{\varphi}$ obtained by the construction on a formula $\varphi$ with criticality $c$ has size $g(c+1,|\varphi|^2 \cdot log\ |\varphi|) \cdot g(c,|\mathcal{K}|^2 \cdot log\ |\mathcal{K}|)$.
\end{theorem}

==> math/theorems/hyperpdl.tex <==
\begin{theorem}
	$HyperPDL-\Delta < H_{\mu}$
\end{theorem}

==> math/theorems/ksynchronousdecidability.tex <==
\begin{theorem}\label{thm:ksynchronousdecidability}
	It is undecidable whether a given $H_{\mu}$ formula is semantically equivalent to a $k$-synchronous formula.
\end{theorem}


==> math/theorems/ksynchronoussatisfiability.tex <==
\begin{theorem}
	The satisfiability problem for linear alternation-free $k$-synchronous $H_{\mu}$ is EXPSPACE-complete.
\end{theorem}

==> math/theorems/linearphaseboundedmodelchecking.tex <==
\begin{theorem}
Model Checking a $k$ phase-bounded $H_{\mu}$ formula with alternation depth $d$ against a Kripke Structure is complete for $\SPACE(g(d+k-1,|\varphi|))$ and $\SPACE(g(d+k-2,|\mathcal{K}|))$.
\end{theorem}


==> math/theorems/mucalculus.tex <==
\begin{theorem}
	$L_{\mu} < H_\mu$
\end{theorem}

==> math/theorems/phaseboundedsatisfiability.tex <==
\begin{theorem}
	The satisfiability problem for alternation-free $k$ phase-bounded $H_{\mu}$ is decidable.
\end{theorem}
\begin{proof}
	Transform formula into a $k$ phase-bounded AAPA and test it for emptiness.
	%\hfill\qed
\end{proof}

==> math/theorems/pushdownexpressivity.tex <==
\begin{theorem}\label{thm:pushdownexpressivity}
For every $n$, there is an alphabet $\Sigma$ and a language over $\Sigma^n$ that is recognisable by a Büchi Pushdown Automaton but not by an AAPA.
\end{theorem}


==> math/theorems/syncexistsforallsatisfiability.tex <==
\begin{theorem}
	The satisfiability problem for the synchronous $\exists^* \forall^*$-fragment of $H_{\mu}^{sync}$ is EXPSPACE-complete.
\end{theorem}

==> math/theorems/synchronouskequivalence.tex <==
\begin{theorem}\label{thm:synchronouskequivalence}
	The automaton $\mathcal{A}_{\varphi}$ obtained by the construction is $\mathcal{K}$-equivalent to $\varphi$.
\end{theorem}

==> math/theorems/synchronoussatisfiability.tex <==
\begin{theorem}
	\begin{enumerate}
	\item The satisfiability problem for linear alternation-free synchronous $H_{\mu}$ is PSPACE-complete.
\item The satisfiability problem for the synchronous $\exists^* \forall^*$-fragment of $H_{\mu}$ is EXPSPACE-complete.
	\end{enumerate}
\end{theorem}


==> sections/introduction/abstractdeadline-abstract.tex <==
\begin{abstract}
Hyperproperties have received increasing attention in the last decade due to their importance e.g. for security analyses. In this paper, we introduce the logic H_\mu for hyperproperties by extending the linear time $\mu$-calculus with quantification over named paths. Unlike prior logics for hyperproperties, H_\mu allows the specification of asynchronous hyperproperties. We prove the satisfiability and the model checking problem for H_\mu to be undecidable. Accordingly, we present approximate satisfiability and model-checking algorithms. These results are achieved via a deep connection between H_\mu and a novel type of alternating asynchronous automata, for which we exhibit corresponding (un-) decidability results.
\end{abstract}



==> sections/main/expressivity.tex <==
\section{Expressivity}\label{sec:expressivity}

\input{math/theorems/mucalculus}
\input{math/proofs/mucalculus}

\input{math/theorems/hyperpdl}
\input{math/proofs/hyperpdl}

\input{math/theorems/asynchronousCTL}
\input{math/proofs/asynchronousCTL}

\tbd{Adapt stuff for branching time}
\tbd{Placement in Hierarchy of Hyperproperties}
\tbd{Comparison to HyperQPTL, S1S(E), MSO(E)/HyperCTL* etc.}
\tbd{$H_{\mu}$ can characterise Basic PA processes up to bisimulation}
\tbd{$H_{\mu}$ can express that $\pi_2$ is the output of a Büchi transducer for $\pi_1$}

